Search for excited $B_c^+$ states

A search is performed in the invariant mass spectrum of the $B_c^{+}\pi^{+}\pi^{-}$ system for the excited $B_c^{+}$ states $B_c(2^{1}S_{0})^+$ and $B_c(2^{3}S_{1})^+$ using a data sample of $pp$ collisions collected by the LHCb experiment at the centre-of-mass energy of $\sqrt{s} = 8 \,{\mathrm{TeV}}$, corresponding to an integrated luminosity of $2 \,{\mathrm{fb^{-1}}}$. No evidence is seen for either state. Upper limits on the ratios of the production cross-sections of the $B_c(2^{1}S_{0})^+$ and $B_c(2^{3}S_{1})^+$ states times the branching fractions of ${B_c(2^{1}S_{0})^+} \to {B_c^{+}\pi^{+}\pi^{-}}$ and ${B_c(2^{3}S_{1})^+} \to {B_c^{*+}\pi^{+}\pi^{-}}$ over the production cross-section of the $B_c^{+}$ state are given as a function of their masses. They are found to be between 0.02 and 0.14 at $95\%$ confidence level for $B_c(2^{1}S_{0})^+$ and $B_c(2^{3}S_{1})^+$ in the mass ranges $[6830, 6890] \,{\mathrm{MeV}}/c^{2}$ and $[6795,6890] \,{\mathrm{MeV}}/c^{2}$, respectively.

==> Makefile <==
MAIN = main

LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib $(MAIN).toc

